Stability of Linear Systems under Extended Weakly-Hard Constraints

Control systems can show robustness to many events, like disturbances and model inaccuracies. It is natural to speculate that they are also robust to sporadic deadline misses when implemented as digital tasks on an embedded platform. This paper proposes a comprehensive stability analysis for control systems subject to deadline misses, leveraging a new formulation to describe the patterns experienced by the control task under different handling strategies. Such analysis brings the assessment of control systems robustness to computational problems one step closer to the controller implementation.

==> evaluation-unstable.tex <==
\begin{table*}
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.06}
\caption{Results obtained for the unstable system $P_2$, when controlled using $C_2$.}\label{table:unstable}
\rowcolors{2}{gray!25}{white}
\begin{center}
\begin{tabular}{|c|clll|clll|clll|clll|}
\hline
% \rowcolor{gray!50}
% &&\multicolumn{3}{c}{Dense $d=1$}&\multicolumn{3}{c}{Sparse $d=1$} &\multicolumn{2}{c}{JSR\_toolbox}\\
% \rowcolor{gray!50}
% \multirow{-2}*{$m$}&\multirow{-2}*{$k$}&$ub$&time&$mb$&$ub$&time&$mb$&$lb$&$ub$\\
\rowcolor{gray!50}
& \multicolumn{4}{c|}{\textbf{Kill and Zero}} & \multicolumn{4}{c|}{\textbf{Kill and Hold}} & \multicolumn{4}{c|}{\textbf{Skip-Next and Zero}} & \multicolumn{4}{c|}{\textbf{Skip-Next and Hold}} \\
\rowcolor{gray!50}
\multicolumn{1}{|c|}{$\overbar{\binom{m}{k}}$} 
& \multicolumn{1}{c}{JSR\cite{vankeerberghen2014jsr}} & \multicolumn{1}{c}{Dense} & \multicolumn{2}{c|}{Sparse}
& \multicolumn{1}{c}{JSR\cite{vankeerberghen2014jsr}} & \multicolumn{1}{c}{Dense} & \multicolumn{2}{c|}{Sparse}
& \multicolumn{1}{c}{JSR\cite{vankeerberghen2014jsr}} & \multicolumn{1}{c}{Dense} & \multicolumn{2}{c|}{Sparse}
& \multicolumn{1}{c}{JSR\cite{vankeerberghen2014jsr}} & \multicolumn{1}{c}{Dense} & \multicolumn{2}{c|}{Sparse} \\
\rowcolor{gray!50}
$m,$ $k$
% kill and zero
& \multicolumn{1}{c}{LB} & \multicolumn{1}{c}{UB} & \multicolumn{1}{c}{UB} & \multicolumn{1}{c|}{$\times$}
% kill and hold
& \multicolumn{1}{c}{LB} & \multicolumn{1}{c}{UB} & \multicolumn{1}{c}{UB} & \multicolumn{1}{c|}{$\times$}
% skip and zero
& \multicolumn{1}{c}{LB} & \multicolumn{1}{c}{UB} & \multicolumn{1}{c}{UB} & \multicolumn{1}{c|}{$\times$}
% skip and hold
& \multicolumn{1}{c}{LB} & \multicolumn{1}{c}{UB} & \multicolumn{1}{c}{UB} & \multicolumn{1}{c|}{$\times$}
\\
\hline
1, 2
& 0.995 & 1.148 & \underline{\textbf{0.995}} & 0.02 % & 0.995 & 1.148 & 1.148 & 0.96
& 0.995 & 1.149 & \underline{\textbf{0.998}} & 0.01 % & 0.995 & 1.149 & 1.149 & 0.97
& 0.995 & \textbf{0.995} & \textbf{0.995} & 1.87
& 0.995 & \textbf{0.995} & \textbf{0.995} & 1.82\\
1, 3
& 0.995  & 1.116 & 1.116$\mathbf{^*}$ & 0.78 % & 0.995  & 1.116 & 1.116 & 0.78
& 0.995  & 1.116 & 1.116$\mathbf{^*}$ & 0.75 % & 0.995  & 1.116 & 1.116 & 0.75
& 0.995  & 1.109$\mathbf{^*}$ & 1.109$\mathbf{^*}$ & 3.00
& 0.995  & 1.110$\mathbf{^*}$ & 1.110$\mathbf{^*}$ & 2.96\\
1, 4
& 0.995 & 1.095 & 1.169$\mathbf{^*}$ & 1.38 % & 0.995  & 1.095 & 1.169 & 1.38
& 0.995 & 1.095 & 1.169$\mathbf{^*}$ & 1.28 % & 0.995  & 1.095 & 1.169 & 1.28
& 0.995 & 1.093$\mathbf{^*}$ & 1.093$\mathbf{^*}$ & 4.05
& 0.995 & 1.093$\mathbf{^*}$ & 1.093$\mathbf{^*}$ & 5.05\\
1, 5
& 0.995  & 1.080 & 1.145$\mathbf{^*}$ & 2.17 % & 0.995  & 1.080 & 1.145 & 2.17
& 0.995  & 1.081 & 1.145$\mathbf{^*}$ & 2.66 % & 0.995  & 1.081 & 1.145 & 2.66
& 0.995  & 1.079$\mathbf{^*}$ & 1.079$\mathbf{^*}$ & 3.90
& 0.995  & 1.080$\mathbf{^*}$ & 1.080$\mathbf{^*}$ & 4.84\\
1, 6
& 0.995 & 1.070 & 1.128$\mathbf{^*}$ & 3.88 % & 0.995  & 1.070 & 1.128 & 3.88
& 0.995 & 1.070 & 1.128$\mathbf{^*}$ & 4.79 % & 0.995  & 1.070 & 1.128 & 4.79
& 0.995 & 1.069$\mathbf{^*}$ & 1.069$\mathbf{^*}$ & 4.04
& 0.995 & 1.070$\mathbf{^*}$ & 1.070$\mathbf{^*}$ & 4.61\\
\hline
2, 3
& 0.995 & 1.162 & \underline{\textbf{0.997}} & 0.01 % & 0.995  & 1.162 & 1.162 & 0.97
& 0.995 & 1.166 & 1.166 & 0.88
& 0.995 & 1.090 & 1.095 & 1.66
& 0.995 & 1.094 & 1.100 & 1.63\\
2, 4
& 0.995 & 1.148 & 1.148$\mathbf{^*}$ & 0.91 % & 0.995  & 1.148 & 1.148 & 0.91
& 0.995 & 1.149 & 1.149 & 0.80
& 0.995 & 1.150 & 1.159 & 2.96
& 0.995 & 1.152 & 1.161 & 4.60\\
2, 5
& 0.995 & 1.131 & 1.195$\mathbf{^*}$ & 1.74 % & 0.995  & 1.131 & 1.195 & 1.74
& 0.995 & 1.132 & 1.195 & 1.87
& 0.995 & 1.134 & 1.142 & 7.79
& 0.995 & 1.135 & 1.143 & 8.70\\
2, 6
& 0.995 & 1.118 & 1.195$\mathbf{^*}$ & 7.49 % & 0.995  & 1.118 & 1.195 & 7.49
& 0.995 & 1.118 & 1.195 & 12.4
& 0.995 & 1.120 & 1.135 & 15.8
& 0.995 & \multicolumn{1}{c}{--} & 1.136 & \multicolumn{1}{c|}{--} \\
\hline
3, 4
& 0.999 & 1.154 & 1.154 & 0.91
& 0.995 & 1.159 & 1.159 & 0.86
& 0.998 & 1.123 & 1.133 & 1.09
& 0.995 & 1.127 & 1.135 & 1.31\\
3, 5
& 0.995 & 1.153 & 1.153 & 0.86
& 0.995 & 1.156 & 1.156 & 0.76
& 0.995 & 1.163 & 1.175 & 2.31
& 0.995 & 1.166 & 1.177 & 3.30\\
3, 6
& 0.995 & 1.144 & 1.195 & 2.67
& 0.995 & 1.146 & 1.218 & 2.76
& 0.995 & \multicolumn{1}{c}{--} & 1.163 & \multicolumn{1}{c|}{--}
& 0.995 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c|}{--}\\
\hline
4, 5
& 1.000 & 1.147 & 1.147 & 0.91
& 0.995 & 1.149 & 1.149 & 0.90
& 1.000 & 1.138 & 1.148 & 1.25
& 0.995 & 1.140 & 1.149 & 1.26\\
4, 6
& 0.995 & 1.148 & 1.148 & 0.71
& 0.995 & 1.153 & 1.153 & 0.60
& 0.995 & 1.166 & 1.178 & 2.12
& 0.995 & \multicolumn{1}{c}{--} & \multicolumn{1}{c}{--} & \multicolumn{1}{c|}{--}\\
\hline
\end{tabular}
\end{center}
\end{table*}


==> tricks.tex <==
% -------------------------------------------------------------------- TRICKS
% bad trick
%\linespread{0.99}

% options for pics
\setlength{\abovecaptionskip}{0pt plus 1pt minus 2pt} %0pt plus
\setlength{\belowcaptionskip}{2pt plus 2pt minus 8pt} %0pt plus
\setlength{\textfloatsep}{2pt plus 1pt minus 2pt} %2pt plus
\setlength{\dbltextfloatsep}{2pt plus 2pt minus 2pt} %2pt plus

% reduce space around equations
\makeatletter
\g@addto@macro\normalsize{%
 \setlength\abovedisplayskip{5pt plus 5pt minus 0pt} %2pt plus
 \setlength\belowdisplayskip{5pt plus 5pt minus 0pt} %2pt plus
 \setlength\abovedisplayshortskip{5pt plus 5pt minus 0pt} %2pt plus
 \setlength\belowdisplayshortskip{5pt plus 5pt minus 0pt} %2pt plus
}
\makeatother

% % reducing space around section headings
% \makeatletter
% \let\origsection\section
% \renewcommand\section{\@ifstar{\starsection}{\nostarsection}}
% \newcommand\nostarsection[1]
% {\sectionprelude\origsection{#1}\sectionpostlude}
% \newcommand\starsection[1]
% {\sectionprelude\origsection*{#1}\sectionpostlude}
%
% \newcommand\sectionprelude{%
%   \vspace{-3pt}
% }
% \newcommand\sectionpostlude{%
%   \vspace{-2pt}
% }
%
% %reducing space around subsection headings
% \let\origsubsection\subsection
% \renewcommand\subsection{\@ifstar{\starsubsection}{\nostarsubsection}}
% \newcommand\nostarsubsection[1]
% {\subsectionprelude\origsubsection{#1}\subsectionpostlude}
% \newcommand\starsubsection[1]
% {\subsectionprelude\origsubsection*{#1}\subsectionpostlude}
%
% \newcommand\subsectionprelude{%
%   \vspace{-4pt}
% }
% \newcommand\subsectionpostlude{%
%   \vspace{-3pt}
% }
% \makeatother

% reducing distance between body and footnotes
%\setlength{\skip\footins}{6pt} %6pt
% -------------------------------------------------------------------- ENDTRICKS

